Near-Optimal Distributed Estimation for a Network of Sensing Units Operating Under Communication Constraints

We study the problem of distributed state estimation in a network of sensing units that can exchange their measurements but the rate of communication between the units is constrained. The units collect noisy, possibly only partial observations of the unknown state; they are assisted by a relay center which can communicate at a higher rate and schedules the exchange of measurements between the units. We consider the task of minimizing the total mean-square estimation error of the network while promoting balance between the individual units' performances. This problem is formulated as the maximization of a monotone objective function subject to a cardinality constraint. By leveraging the notion of weak submodularity, we develop an efficient greedy algorithm for the proposed formulation and show that the greedy algorithm achieves a constant factor approximation of the optimal objective. Our extensive simulation studies illustrate the efficacy of the proposed formulation and the greedy algorithm.

==> AlgOld.tex <==
In this section, we propose a randomized greedy algorithm for sensor scheduling in Kalman filtering setting and analyze its performance. %\footnote{Some proofs have been omitted for brevity and are available in the arXiv version in \cite{ma}.}. 
It is straightforward to see that scheduling sensors to minimize the MSE 
objective %\ref{eq:mse} 
at each time step $t$ is equivalent to solving the maximization
\begin{equation}\label{eq:sensor}
\begin{aligned}
& \underset{S}{\text{max}}
\quad \mathrm{Tr}\left(\P_{t|t-1}-\F_S^{-1}\right)
& \text{s.t.}\hspace{0.5cm}  S \subset [n], \phantom{k}|S|=k.
\end{aligned}
\end{equation}
%where $\F_S = \P_{t|t-1}^{-1}+\sigma^{-2}\sum_{i\in S}\a_i(t)\a_i(t)^\top$. 
By defining $X = [n]$ and $\mathcal{I} = \{S \subset X| |S|=k\}$, it is easy to see that $\mathcal{M}=(X,\mathcal{I})$ is a uniform matroid. Let $f(S)$ denote the objective function of \ref{eq:sensor}.
%, i.e., the shifted additive inverse of the estimator's mean square error.
Then we can show (details omitted for brevity) that $f(S)$ is a monotonically increasing set function, $f(\emptyset)=0$, and 
\begin{equation}\label{eq:mg}
f_j(S) = \frac{\a_j(t)^\top\F_S^{-2}\a_j(t)}{\sigma^{2}+\a_j(t)^\top\F_S^{-1}\a_j(t)},
\end{equation}
\begin{equation}\label{eq:upf}
\F_{S \cup\{j\}}^{-1} = \F_{S}^{-1}-\frac{\F_{S}^{-1}\a_{j}(t)\a_{j}(t)^\top\F_{S}^{-1}}{\sigma^2+\a_{j}(t)^\top\F_{S}^{-1}\a_{j}(t)}.
\end{equation}
% Proposition \oldref{p:mono} below states that $f(S)$ is monotone and proposes a recursive scheme to efficiently compute the marginal gain of querying a sensor.
% \begin{proposition}\label{p:mono}
% $f(S)$ is a monotonically increasing set function, $f(\emptyset)=0$, and 
% \begin{equation}\label{eq:mg}
% f_j(S) = \frac{\a_j(t)^\top\F_S^{-2}\a_j(t)}{\sigma^{2}+\a_j(t)^\top\F_S^{-1}\a_j(t)}.
% \end{equation}
% \begin{equation}\label{eq:upf}
% \F_{S \cup\{j\}}^{-1} = \F_{S}^{-1}-\frac{\F_{S}^{-1}\a_{j}(t)\a_{j}(t)^\top\F_{S}^{-1}}{\sigma^2+\a_{j}(t)^\top\F_{S}^{-1}\a_{j}(t)}
% \end{equation}
% \end{proposition}
% \begin{proof}
% See Appendix 
% %\oldref{pf:mono}.
% I in \cite{ma}.
% \end{proof}

The combinatorial optimization problem in \ref{eq:sensor} is NP-hard as one needs to exhaustively search over all schedules of $k$ sensors to find the optimal solution. 
An approximate solution, i.e., a schedule of sensors that results in a sub-optimal MSE,  can be found by the following SDP relaxation (see Appendix 
%\oldref{pf:sdp} 
II in \cite{ma} 
for the derivation),
\begin{equation}\label{sdp}
\begin{aligned}
& \underset{\z,\Y}{\text{min}}
\quad \mathrm{Tr}(\Y)\\
& \text{s.t.}\hspace{0.5cm}  0\leq z_i \leq 1, \phantom{k} \forall i\in [n] \\ 
& \hspace{0.9cm} \sum_{i=1}^n z_i =k\\
& \hspace{0.9cm} 
\begin{bmatrix}
    \Y& \I\\
    \I & \P_{t|t-1}^{-1}+\sigma^{-2}\sum_{i=1}^n z_i\a_i(t)\a_i(t)^\top
\end{bmatrix} \succeq \mathbf{0}.
\end{aligned}
\end{equation}
%=================================== ALGORITHM 1
\renewcommand\algorithmicdo{}	% removes "DO" from for loops
\begin{algorithm}
\caption{Randomized Greedy Sensor Scheduling}
\label{alg:greedy}
\begin{algorithmic}[1]
    \STATE \textbf{Input:}  $\P_{t|t-1}$, $\A_t$, $k$, $\epsilon$.
    \STATE \textbf{Output:} Subset $S_t\subseteq [n]$ with $|S_t|=k$.
    \STATE Initialize $S_t^{(0)} =  \emptyset$, $\F_{S_t^{(0)}}=\P_{t|t-1}^{-1}$.
	\FOR{$i = 0,\dots, k-1$}
			\STATE Choose $R$ by sampling $s=\frac{n}{k}\log{(1/\epsilon)}$ indices uniformly at random from $[n]\backslash S_t^{(i)}$.\vspace{0.2cm}
            \STATE $i_s = \argmax_{j\in R} \frac{\a_j(t)^\top\F_{S_t^{(i)}}^{-2}\a_j(t)}{\sigma^{2}+\a_j(t)^\top\F_{S_t^{(i)}}^{-1}\a_j(t)}$.\vspace{0.2cm}
            \STATE Set $S_t^{(i+1)}= S_t^{(i)}\cup \{i_s\}$.\vspace{0.2cm}
            \STATE $\F_{S_t^{(i+1)}}^{-1} = \F_{S_t^{(i)}}^{-1}-\frac{\F_{S_t^{(i)}}^{-1}\a_{i_s}(t)\a_{i_s}(t)^\top\F_{S_t^{(i)}}^{-1}}{\sigma^2+\a_{i_s}(t)^\top\F_{S_t^{(i)}}^{-1}\a_{i_s}(t)}$.
	\ENDFOR
	\RETURN $S_t = S_t^{(k)}$.
\end{algorithmic}
\end{algorithm}
%===================================
The complexity of the SDP algorithm scales as ${\cal O}(n^3)$ which is infeasible in practice. Furthermore, there is no guarantee on the achievable MSE performance of the SDP relaxation. When the number of sensors in a network and the size of the state vector $\x(t)$ are relatively large, even the greedy algorithm proposed in \cite{shamaiah2010greedy} may be computationally prohibitive. To provide practical feasibility, inspired by the recent work in \cite{mirzasoleiman2014lazier} for submodular objectives, we propose a computationally efficient randomized greedy algorithm (see Algorithm \oldref{alg:greedy}) that finds an approximate solution to \ref{eq:sensor} with a guarantee on the expected MSE. Algorithm \oldref{alg:greedy} performs the task of sensor scheduling in the following way. At each iteration of the algorithm, a subset $R$ of size $s$ is sampled uniformly at random and without replacement from the set of sensors. The marginal gain provided by each of these $s$ sensors to the objective function is computed using \ref{eq:mg}, and the one yielding the highest marginal gain is added to the set of selected sensors. Then the efficient recursive formula in \ref{eq:upf} is used to update $\F_S^{-1}$ so that it can be used in the next iteration. This procedure is repeated $k$ times.

\textit{Remark 1:} The parameter $\epsilon$ in Algorithm \oldref{alg:greedy}, $e^{-k}\leq\epsilon<1$, denotes a predefined constant that is chosen to strike a desired balance between performance and complexity. When $\epsilon = e^{-k}$, each iteration includes all of the non-selected sensors in $R$ and Algorithm \oldref{alg:greedy} coincides with the classical greedy scheme. However, as $\epsilon$ approaches $1$, $|R|$ and thus the overall computational complexity decreases. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Performance Analysis of the Proposed Scheme}
In this section, we analyze Algorithm \oldref{alg:greedy} and in Theorem \oldref{thm:card} provide a bound on the performance of the proposed randomized greedy scheme when applied to finding an approximate solution to the maximization problem in \ref{eq:sensor}.
% Before stating the main results, we first provide two lemmas. Lemma \oldref{lem:curv} upper-bounds the difference between the values of the objective corresponding to two sets having different cardinalities while Lemma \oldref{lem:rand} provides a lower bound on the expected marginal gain.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{lemma}\label{lem:curv}
% \textit{Let $\{{\cal C}_l\}_{l=1}^{n-1}$ be the element-wise curvatures of $f(S)$. Let $S$ and $T$ be any schedules of sensors such that $S\subset T \subseteq [n]$ with $|T\backslash S|=r$. Then, it holds that
% \begin{equation}
% f(T)-f(S)\leq  C(r)\sum_{j\in T\backslash S}f_j(S),
% \end{equation}
% where $ C(r)=\frac{1}{r}(1+\sum_{l=1}^{r-1}{\cal C}_l)$.}
% \end{lemma}
% \begin{proof}
% See Appendix 
% %\oldref{pf:curv}.
% III in \cite{ma}.
% \end{proof}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{lemma}\label{lem:rand}
% \textit{Let $S_t^{(i)}$ be the set of selected sensors at the end of the $i\ts{th}$ iteration of Algorithm \oldref{alg:greedy}. Then
% \begin{equation}
% \E\left[f_{(i+1)_s}(S_t^{(i)})|S_t^{(i)}\right]\geq \frac{1-\epsilon^{\beta}}{k}\sum_{j\in O_t\backslash S_t^{(i)}}f_j(S_t^{(i)}),
% \end{equation}
% where $O_t$ is the set of optimal sensors at time $t$, $i_s$ is the index of the selected sensor at the $i\ts{th}$ iteration, and $\beta\geq1$ is a constant that depends on $n$, $k$, and $\epsilon$.}
% \end{lemma}
% \begin{proof}
% See Appendix 
% %\oldref{pf:rand}.
% IV in \cite{ma}.
% \end{proof}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The theorem states that %Algorithm \oldref{alg:greedy} provides an approximate solution to the sensor scheduling problem. In particular, 
if $f(S)$ is characterized by a bounded maximum element-wise curvature, Algorithm \oldref{alg:greedy} returns a subset of sensors yielding an objective value that is on average within a multiplicative factor of the objective value achieved by the optimal schedule.

\begin{theorem}\label{thm:card}
\textit{Let $\mathcal{C}_{max}$ be the maximum element-wise curvature of $f(S)$, i.e., the objective function of sensor scheduling problem in \ref{eq:sensor}. Let $S_t$ denote the schedule of sensors selected by Algorithm \oldref{alg:greedy} at time $t$, and let $O_t$ be the optimum solution of \ref{eq:sensor} such that $|O_t|=k$. Then $f(S_t)$ is on expectation a multiplicative factor away from $f(O_t)$. That is,}
\begin{equation}\label{eq:card}
\E\left[f(S_t)\right]\geq \left(1-e^{-\frac{1}{c}}-\frac{\epsilon^\beta}{c}\right) f(O_t),
\end{equation}
\textit{where $c=1$ if ${\cal C}_{\max}\leq 1$ and $c={\cal C}_{\max}$ if ${\cal C}_{\max}\geq 1$, $e^{-k}\leq\epsilon<1$, and $\beta\geq 1$. Furthermore, the computational complexity of Algorithm \oldref{alg:greedy} is ${\cal O}(nm^2\log(\frac{1}{\epsilon}))$ where $n$ is the total number of sensors and $m$ is the dimension of $\x(t)$.}
\end{theorem}
\begin{proof}
Consider $S_t^{(i)}$, the set generated at $i\ts{th}$ iteration of Algorithm \oldref{alg:greedy}. 
Employing Lemma 1 in \cite{ma} %\oldref{lem:curv} 
with $S=S_t^{(i)}$ and $T=O_t\cup S_t^{(i)}$, and using monotonicity of $f$ yields
\begin{equation*}
\begin{aligned}
\frac{f(O_t)-f(S_t^{(i)})}{\frac{1}{r}\left(1+\sum_{l=1}^{r-1}{\cal C}_l\right)}%&\leq \frac{f(O_t\cup S_t^{(i)})-f(S_t^{(i)})}{\frac{1}{r}\left(1+\sum_{l=1}^{r-1}{\cal C}_l\right)}\\
&\leq  \sum_{j\in O_t\backslash S_t^{(i)}}f_j(S_t^{(i)}),
\end{aligned}
\end{equation*}
where $|O_t\backslash S_t^{(i)}|=r$. Now, using Lemma 2 in \cite{ma} %\oldref{lem:rand} 
we obtain
\begin{equation*}
\E\left[f_{(i+1)_s}(S_t^{(i)})|S_t^{(i)}\right]\geq \left(1-\epsilon^{\beta}\right)\frac{f(O_t)-f(S_t^{(i)})}{\frac{k}{r}\left(1+\sum_{l=1}^{r-1}{\cal C}_l\right)},
\end{equation*}
where $\beta=1+ \max\{0,\frac{s}{2n}-\frac{1}{2(n-s)}\}$.
Applying the law of total expectation results in
\begin{equation}\label{eq:th1-1}
\begin{aligned}
\E\left[f_{(i+1)_s}(S_t^{(i)})\right]%&=\E\left[f(S_t^{(i+1)})-f(S_t^{(i)})\right]\\
&\geq \left(1-\epsilon^{\beta}\right)\frac{f(O_t)-\E\left[f(S_t^{(i)})\right]}{\frac{k}{r}\left(1+\sum_{l=1}^{r-1}{\cal C}_l\right)}.
\end{aligned}
\end{equation}
Using the definition of ${\cal C}_{\max}$ we obtain 
\begin{equation*}
\frac{1}{r}\left(1+\sum_{l=1}^{r-1}{\cal C}_l\right)\leq \frac{1}{r}(1+(r-1){\cal C}_{\max}) =g(r).
\end{equation*}
One can verify, e.g., by taking the derivative, that $g(r)$ is decreasing (increasing) with respect to $r$ if ${\cal C}_{\max}<1$ (${\cal C}_{\max}>1$). Let $c=1$ if ${\cal C}_{\max}\leq 1$ and $c={\cal C}_{\max}$ if ${\cal C}_{\max}\geq 1$. Then 
\begin{equation}\label{eq:th1-2}
\frac{1}{r} \left(1+\sum_{l=1}^{r-1}{\cal C}_l\right)\leq \frac{1}{r}(1+(r-1){\cal C}_{\max}) \leq c.
\end{equation}
Hence, combining \ref{eq:th1-1} and \ref{eq:th1-2} yields
\begin{equation*}
\E\left[f(S_t^{(i+1)})-f(S_t^{(i)})\right]\geq \frac{1-\epsilon^\beta}{kc}\left(f(O_t)-\E\left[f(S_t^{(i)})\right]\right).
\end{equation*}
By induction and due to the fact that $f(\emptyset) = 0$, 
\begin{equation*}
\E[f(S_t)]\geq \left(1-\left(1-\frac{1-\epsilon^\beta}{kc}\right)^k\right)f(O_t).
\end{equation*}
Finally, using the fact that $(1+x)^y\leq e^{xy}$ for $y>0$ and  the easily verifiable fact that $e^{ax}\leq 1+axe^a$ for $0<x<1$, 
\begin{equation*}
\begin{aligned}
\E[f(S_t)]%&\geq \left(1-e^{-\frac{1-\epsilon^\beta}{c}}\right)f(O_t)\\
&\stackrel{}{\geq} \left(1-e^{-\frac{1}{c}}-\frac{\epsilon^\beta}{c}\right)f(O_t).
\end{aligned}
\end{equation*}
To take a closer look at computational complexity of Algorithm \oldref{alg:greedy}, note that step 6 costs $\mathcal{O}(\frac{n}{k}m^2\log(\frac{1}{\epsilon}))$ as one needs to compute $\frac{n}{k}\log(\frac{1}{\epsilon})$ marginal gains, each with complexity ${\cal O}(m^2)$. Step 8 requires ${\cal O}(m^2)$ arithmetic operations. Since there are $k$ such iterations, running time of Algorithm \oldref{alg:greedy} is ${\cal O}(nm^2\log(\frac{1}{\epsilon}))$. This completes the proof.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We can now establish a bound on the achievable MSE (denoted by $\mathrm{MSE}_{S_t}$) by using the definition of $f(S)$:
\begin{equation}\label{eq:card1}
\E\left[\mathrm{MSE}_{S_t}\right]\leq \alpha \mathrm{MSE}_{o} + (1-\alpha) \mathrm{Tr}(\P_{t|t-1}),
\end{equation}
where $\alpha =(1-e^{-\frac{1}{c}}-\frac{\epsilon}{c})$, and  $\mathrm{MSE}_{o}$  denotes the optimal mean square estimation error.

% Using the definition of $f(S)$ we obtain Corollary \oldref{col:mse} stating that, at each time step, the achievable mean-square error in \ref{eq:mse} obtained by forming an estimate using sensors selected by the randomized greedy algorithm is within a factor of the optimal mean-square error.

% \begin{corollary}\label{col:mse}
% \textit{Let $\mathcal{C}_{max}$ be the maximum element-wise curvature of $f(S)$, the objective function of the sensor scheduling problem \ref{eq:sensor}. Let $\alpha =(1-e^{-\frac{1}{c}}-\frac{\epsilon}{c})$ where $c=1$ if ${\cal C}_{\max}\leq 1$ and $c={\cal C}_{\max}$ if ${\cal C}_{\max}\geq 1$, and $e^{-k}\leq\epsilon<1$. Let $\mathrm{MSE}_{S_t}$ denote the mean-square estimation error obtained by forming an estimate using information provided by the sensors selected by Algorithm \oldref{alg:greedy} at time $t$, and let $\mathrm{MSE}_{o}$ be the optimal mean-square error formed using information collected by optimum solution of \ref{eq:sensor}. Then the expected $\mathrm{MSE}_{S_t}$ is bounded as}
% \begin{equation}\label{eq:card1}
% \E\left[\mathrm{MSE}_{S_t}\right]\leq \alpha \mathrm{MSE}_{o} + (1-\alpha) \mathrm{Tr}(\P_{t|t-1}).
% \end{equation}
% \end{corollary}

\textit{Remark 2:} 
% Since the proposed scheme is a randomized algorithm, Theorem \oldref{thm:card} and Corollary \oldref{col:mse} state that the expected MSE associated with the solution returned by Algorithm \oldref{alg:greedy} is a multiplicative factor $\alpha$ away from the optimal MSE. 
Notice that, as we expect, $\alpha$ is decreasing in both $c$ and $\epsilon$. 
If $f(S)$ is characterized by a small curvature, then $f(S)$ is nearly submodular and randomized greedy algorithm delivers a near-optimal scheduling. As we decrease $\epsilon$, a larger subset of sensors is evaluated each time. Therefore, $\alpha$ increases which in turn results in a better approximation. %factor.

\textit{Remark 3:} The computational complexity of the greedy method proposed in \cite{shamaiah2010greedy} is ${\cal O}(knm^2)$. Hence, our proposed scheme provides a reduction in complexity by $k\slash \log(\frac{1}{\epsilon})$ which may be particularly beneficial in large-scale networks. 


Recall that $f(S)$ is not submodular \cite{olshevsky2017non}. However, in the statement of Theorem \oldref{thm:card} we assumed that it has a bounded maximum element-wise curvature. In Theorem \oldref{thm:curv} below, using concentration of measure inequalities such as matrix Bernstein inequality \cite{tropp2015introduction}, we assert that a probabilistic theoretical upper bound on the maximum element-wise curvature of $f(S)$ exists in scenarios where at each time step the measurement vectors $\a_j(t)$'s are i.i.d. random vectors. 

\begin{theorem}\label{thm:curv}
\textit{Let $\mathcal{C}_{max}$ be the maximum element-wise curvature of $f(S)$, i.e., the objective function of sensor scheduling problem. Let $\a_j(t)$'s be independent zero-mean random vectors with covariance matrix $\sigma_h^2\I_m$ such that for all $j$, $\|\a_j(t)\|_2^2\leq C$. Then, for all $q>0$ with probability 
\begin{equation} \label{eq:psuc}
p\geq 1-m\exp\left(\frac{-q^2\slash 2}{(C-\sigma_h^2)(n\sigma_h^2+q\slash 3)}\right)
\end{equation}
it holds that 
\begin{equation}\label{eq:phic}
\mathcal{C}_{max} \leq \frac{\lambda_{max}(\P_{t|t-1})^{2}(\sigma^{2}+\lambda_{max}(\P_{t|t-1})C)}{\phi^{2}(\sigma^{2}+\phi C)},
\end{equation}
where 
\begin{equation}\label{eq:phi}
\phi \geq \left(\frac{1}{\lambda_{min}(\P_{t|t-1})}+\frac{n\sigma_h^2+q}{\sigma^2}\right)^{-1}.
\end{equation}}
\end{theorem}
\textit{Remark 4:} The setting of i.i.d. random vectors described in Theorem \oldref{thm:curv} arises in scenarios where sketching techniques, such as random projections are used to reduce dimensionality of the measurement equation \cite{berberidis2016data}. 

\textit{Remark 5:} The conditions stated in Theorem \oldref{thm:curv} can be interpreted as follows.  For sufficiently large $m  $, and when $\sigma_h^2 = \frac{1}{m}$, we can approximate $C \approx 1$. Assume $\phi \geq \lambda_{max}\slash \delta$ for some $\Delta>1$. Let $\mathrm{SNR} = \lambda_{max}(\P_{t|t-1}) \slash \sigma^2$ and $\kappa = \lambda_{max}(\P_{t|t-1}) \slash \lambda_{min}(\P_{t|t-1})>1$ be the condition number of $\P_{t|t-1}$. With some numerical approximations one can show that if
\begin{equation*}
\Delta \geq \kappa +c_1\frac{n}{m}\mathrm{SNR},
\end{equation*}
with probability $p>1-m\exp(-\frac{n}{m}c_2)$, $\mathcal{C}_{max} \leq \Delta^3$, for some $c_1$, $c_2>0$. Hence, informally, Theorem \oldref{thm:curv} states that for a well-conditioned $\P_{t|t-1}$, curvature of $f(S)$ is small, implying weak-submodularity of $f(S)$.
% \begin{proof}
% See Appendix 
% %\oldref{pf:thm:curv}.
% V in \cite{ma}.
% \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We now consider widely used examples of measurement vectors to show practicality of the results of Theorem \oldref{thm:curv}.
% \begin{enumerate}
% \item {\it Multivariate Gaussian measurement vectors:} Let $\a_j(t) \sim \mathcal{N}(0,\frac{1}{m}\I_m)$ for all $j$. It is easy to show that $\E[\|\a_j(t)\|_2^2] = 1$ for all $j$. Furthermore, it can be shown that $\|\a_j(t)\|_2^2$ is with high probability distributed around its expected value. Therefore, for this case,  $\sigma_h^2 = \frac{1}{m}$ and $C = 1$.
% \item {\it Centered Bernoulli measurement vectors:} Let each entry of $\a_j(t)$ be set to $\pm \frac{1}{\sqrt{m}}$ with equal probability. Therefore, $\|\a_j(t)\|_2^2=1 = C $. Additionally, $\sigma_h^2 = \frac{1}{m}$ since the entries of $\a_j(t)$ are i.i.d. zero-mean random variables with variance $\frac{1}{m}$.
% %\item {\it Deterministic orthonormal measurement vectors: }
% \end{enumerate}
% Extension 1: Lazy evaluation
% Extension 2: Design sensors with a given tolerance
% Both for journal version


==> IntroOld.tex <==
Large-scale sensor networks have drawn considerable attention in recent years \cite{joshi2009sensor,shamaiah2010greedy,tzoumas2016sensor,tzoumas2016scheduling,tzoumas2016near,carlone2016attention}. In such a network, due to various practical considerations and limitations on resources including computational and communication constraints, the data center which aggregates information typically queries only a small subset of the available sensors. This scenario describes many problems in control systems, signal processing, and machine learning, including sensor selection for Kalman filtering \cite{nordio2015sensor,shamaiah2010greedy}, batch state estimation and stochastic process estimation \cite{tzoumas2016scheduling,tzoumas2016near}, minimal actuator placement \cite{tzoumas2015minimal}, subset selection in machine learning \cite{mirzasoleiman2014lazier}, voltage control and meter placement in power networks \cite{damavandi2015robust,gensollen2016submodular,liu2016towards}, and sensor scheduling in wireless sensor networks \cite{shamaiah2012greedy,nordio2015sensor}.

Optimal sensor selection requires finding solution to a computationally challenging combinatorial optimization problem, which has motivated development of heuristics and approximate algorithms. In \cite{joshi2009sensor}, sensor selection is formulated as the maximization (minimization) of the $\log \det$ of the Fisher information matrix (error covariance matrix) and a semidefinite programming (SDP) relaxation is proposed. The computational complexity of the SDP relaxation is cubic in the number of sensors in the network which limits practical feasibility of this scheme. Additionally, the SDP relaxation does not come with any performance guarantees. To overcome these drawbacks, Shamaiah et al. \cite{shamaiah2010greedy} proposed a greedy algorithm for the $\log \det$ maximization formulation of the sensor selection problem whose complexity is significantly lower than that of the SDP relaxation. Since the $\log \det$ of the Fisher information matrix is a monotone submodular function, the greedy scheme in \cite{shamaiah2010greedy} is a $(1-1\slash e)$-approximation algorithm. More recently, the greedy algorithm for $\log \det$ maximization was employed and analyzed in a number of practical settings \cite{tzoumas2016scheduling,tzoumas2015minimal,tzoumas2016near,summers2016submodularity}. 
%For instance, Tzoumas et al. \cite{tzoumas2016sensor} extended the result of \cite{shamaiah2010greedy} by showing that $\log \det$ of the error covariance matrix of the Kalman filter in presence of process noise is supermodular. 
However, even though $\log \det$ is related to the volume of the $\eta$-confidence ellipsoid, it is not explicitly related to the mean square error (MSE) which is often the performance measure of interest in sensor scheduling and state estimation problems. The MSE, i.e., the trace of the error covariance matrix, is not supermodular \cite{krause2008near,olshevsky2017non,summers2016submodularity}. Therefore, the search for an approximation algorithm with performance guarantees on the estimator's achievable MSE remains an open research problem.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Greedy Algorithms for Combinatorial Optimization}
The success of submodular maximization in sensor selection applications is due to the extensive prior work in designing approximation algorithms for combinatorial optimization problems. Nemhauser et al.\cite{nemhauser1978analysis} showed that the greedy algorithm provides a $(1-1/e)$-approximation to maximizing a monotone submodular set function under cardinality constraint. 
% They extended their work to the nonuniform matroid constraint and showed that the greedy algorithm achieves a $1/(P+1)$-approximation over the intersection of $P$ matroids \cite{fisher1978analysis}.
% A ($\frac{1-e^{-c}}{c}$)-approximation algorithm for the monotone submodular function maximization under any matroid constraint was proposed in \cite{vondrak2010submodularity}. 
% {\color{blue}{The curvature in \cite{vondrak2010submodularity} is measured with respect to the optimum. Given the NP-completeness of the problem, finding the curvature with respect to the optimum remains challenging.}} 
% A local search method proposed in \cite{filmus2014monotone} provides a ($\frac{1-e^{-c}}{c}$)-approximation for monotone submodular maximization over matroid constraints.
% Sviridenko et al. \cite{sviridenko2015optimal} introduced a ($1-c/e-\epsilon$)-approximation algorithm for the maximization of monotone increasing submodular functions and a ($1+\frac{c}{1-c}.e^{-1}+\frac{1}{1-c}O(\epsilon)$)-approximation algorithm for the minimization of monotone decreasing supermodular functions
% subject to a single matroid constraint. The approximation ratio there
% improved the previous ($\frac{1-e^{-c}}{c}$)-approximation of \cite{vondrak2010submodularity}. 
In \cite{mirzasoleiman2014lazier}, a ($1-1/e-\epsilon$)-approximation stochastic-greedy algorithm is developed for the maximization of monotone increasing submodular functions. Recently, Wang \etal \cite{wang2016approximation} analyzed the performance of the greedy algorithm in the general setting where the function is monotone non-decreasing, but not necessarily submodular. They defined an elemental curvature $\alpha$ and showed that the greedy algorithm provides a $(\frac{1}{1+\mu(\alpha)})$-approximation under a general matroid constraint.
% , where $\mu=\alpha$ if $0\leq \alpha \leq 1$ and $\mu=\frac{\alpha^K(1-\alpha^K)}{K(1-\alpha)}$ if $\alpha>1$ ($K$ denotes the rank of the matroid). 
However, determining the elemental curvature is itself an NP-hard task. Therefore, finding an explicit approximation factor for the settings where the objective function is not supermodular, e.g., trace of the error covariance matrix in sensor scheduling,
%for state estimation via Kalman filtering, 
remains a challenge.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Contribution}
Processing massive amounts of data collected by large-scale networks may be challenging even when relying on greedy algorithms. Moreover, the objective function that is typically of interest in sensor scheduling applications, the MSE, is not submodular (or supermodular, in case one considers the minimization formulation of the problem). Hence, the performance guarantees for the greedy scheme derived in \cite{nemhauser1978analysis,fisher1978analysis} no longer hold. In this paper, we address these challenges by making the following contributions:
\begin{itemize}
\item We formulate the sensor scheduling task as the problem of maximizing a monotone objective function directly related to the MSE of the estimator.
\item We propose a randomized greedy algorithm and, by introducing the notion of curvature $c$, find a bound on the expected MSE of the state estimate formed by the Kalman filter that uses the measurements of the sensors selected by the randomized greedy algorithm.
\item We derive a probabilistic bound on the curvature $c$ for the cases where the measurements are i.i.d. random vectors with bounded $\ell_2$-norm,
%. These results are relevant 
 e.g., in scenarios of randomly-sketched measurement vectors \cite{berberidis2016data}.
\item In simulation studies, we illustrate that our proposed randomized greedy algorithm significantly outperforms greedy and SDP relaxation methods in terms of runtime while providing essentially the same or improved MSE. 
\end{itemize}
%The rest of the paper is organized as follows. Section \oldref{sec:sys} explains the system model and reviews some related concepts. In Section \oldref{sec:alg}, we introduce the randomized greedy algorithm and analyze its performance. Section \oldref{sec:sim} presents the simulation results while the concluding remarks are stated in Section \oldref{sec:concl}.% \footnote{MATLAB implementation of the proposed algorithm in this paper is freely available at \url{https://github.com/realabolfazl/RGSS}.}


==> PreOld.tex <==
We briefly summarize the notation used in the paper. Bold capital letters refer to matrices and bold lowercase letters represent vectors. $\A_{ij}$ denotes the $(i,j)$ entry of $\A$, $\a_j$ is the $j\ts{th}$ row of $\A$, $\A_{S}$ is a submatrix of $\A$ that contains rows indexed by set $S$, and $\lambda_{max}(\A)$
and $\lambda_{min}(\A)$ are maximum and minimum eigenvalues of $\A$, respectively. Spectral norm ($\ell_2$-norm) of a matrix is denoted by $\|.\|$. $\I_n \in \R^{n\times n}$ is the identity matrix. Moreover, let $[n] := \{1,2,\dots,n\}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Combinatorial Optimization with Matroid Constraint}
This subsection overviews definitions that are essential in the analysis of the randomized greedy algorithm and then introduces the general combinatorial optimization problem studied in the paper.
\begin{definition}
\label{def:unif}
A set function $f:2^X\rightarrow \mathbb{R}$ is monotone non-decreasing if $f(S)\leq f(T)$ for all $S\subseteq T\subseteq X$.
\end{definition}
\begin{definition}
\label{def:submod}
Set function $f:2^X\rightarrow \mathbb{R}$ is submodular if 
\begin{equation*}
f(S\cup \{j\})-f(S) \geq f(T\cup \{j\})-f(T)
\end{equation*}
for all subsets $S\subseteq T\subset X$ and $j\in X\backslash T$. The term $f_j(S)=f(S\cup \{j\})-f(S)$ is the marginal value of adding element $j$ to set $S$.
\end{definition}

A closely related concept to submodularility is the notion of curvature of a set function that quantifies 
how close the function is to being submodular \cite{das2011submodular}. Here, we define the element-wise curvature.
\begin{definition}
 The element-wise curvature of a monotone non-decreasing function $f$ is defined as
 \begin{equation*}
 {\cal C}_l=\max_{(S,T,i)\in \mathcal{X}_l}{f_i(T)\slash f_i(S)},
 \end{equation*}
where $\mathcal{X}_l = \{(S,T,i)|S \subset T \subset X, i\in X \backslash T, |T\backslash S|=l,|X|=n\}$. Furthermore, the maximum element-wise curvature is given by ${\cal C}_{\max}=\max_{l=1}^{n-1}{{\cal C}_l}$.
\end{definition}
Note that a set function is submodular iff ${\cal C}_{\max} \le 1$.

\begin{definition}
Let $X$ be a finite set and let $\mathcal{I}$ be a collection of subsets of $X$. The pair $\mathcal{M}=(X,\mathcal{I})$ is a matroid if the following properties hold: 
\begin{itemize}
\item Hereditary property. If $T\in \mathcal{I}$, then $S\in \mathcal{I}$ for all $S\subseteq T$.
\item Augmentation property. If $S,T\in \mathcal{I}$ and $\abs{S}<\abs{T}$, then there exists $e\in T\backslash S$ such that $S\cup \{e\}\in \mathcal{I}$.
\end{itemize}
The collection $\mathcal{I}$ is called the set of independent sets of the matroid $\mathcal{M}$. A maximal independent set is a basis. It is easy to show that all the bases of a matroid have the same cardinality.
\end{definition}
It can be shown that a cardinality constraint over a set defines a matorid. Let $X$ to denote a set and $\mathcal{I} = \{S \in X | |S|=k\}$. The resulting matroid, i.e., $\mathcal{M}=(X,\mathcal{I})$ is called a uniform matroid.


Given a monotone non-decreasing set function $f:2^X\rightarrow \mathbb{R}$ with $f(\emptyset)=0$, and a matroid $\mathcal{M}=(X,\mathcal{I})$, we
are interested in the combinatorial problem
\begin{equation}\label{eq:fmax}
\max_{S \in \mathcal{I}} f(S).
\end{equation}
Next, we state the problem of sensor scheduling for Kalman filtering and show how to formulate it as a maximization problem described by \ref{eq:fmax}. Then, we present a randomized greedy algorithm to approximately solve this optimization problem and provide its performance guarantees.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sensor Scheduling for Kalman Filtering}
Consider a linear time-varying dynamical system and its measurement model,
\begin{equation}\label{eq:sys}
\begin{aligned}
\x(t+1) &= \H(t)\x(t)+\w(t) \\
\y(t) &= \A(t)\x(t)+\v(t),
\end{aligned}
\end{equation}
where $\x(t) \in \R^m$ is the state vector, $\y(t) \in 
\R^n$ is the measurement vector, $\w(t)$ and $\v(t)$ 
are zero-mean Gaussian noises with covariances
$\mathbf{Q}(t)$ and $\mathbf{R}(t)$, respectively, $\H(t) 
\in  \R^{m \times m}$ is the state transition
matrix and $\A(t) \in  \R^{n \times m}$ is the matrix 
whose rows at time $t$ are the measurement vectors 
$\a_i(t) \in \R^m$. We assume that the states $\x(t)$ are uncorrelated with $\w(t)$ and $\v(t)$. In addition, for simplicity of exposition we assume that $\x(0) \sim {\cal N}(0, \mathbf{\Sigma}_x)$, $\mathbf{Q}(t)=\sigma^2\I_m$, and $\mathbf{R}(t)=\sigma^2\I_n$.

Due to limited resources, fusion center aims to select $k$ out of $n$ sensors and use their measurements to estimate the state vector $\x(t)$ by minimizing the MSE in the Kalman filtering setting. Note that we assume that the measurement vectors $\a_i(t)$ are available at the fusion center.

Let $\P_{t|t-1}$ and $\P_{t|t}$ be the prediction and filtered error covariance at
time instant $t$, respectively. Then
\begin{equation*}
\begin{aligned}
\P_{t|t-1} &= \H(t)\P_{t-1|t-1}\H(t)^\top+\mathbf{Q}(t), \\
\P_{t|t} &= \left(\P_{t|t-1}^{-1}+\A_{S_{t}}(t)^\top\mathbf{R}_{S_{t}}(t)^{-1}\A_{S_{t}}(t)\right)^{-1},
\end{aligned}
\end{equation*}
where $S_{t}$ is the set of selected sensors at time $t$ and $P_{0|0}=\mathbf{\Sigma}_x$. Since $\mathbf{R}(t)=\sigma^2\I_n$ and the measurements are uncorrelated across sensors, it holds that
\begin{equation*}
\begin{aligned}
\P_{t|t} = \left(\P_{t|t-1}^{-1}+\sigma^{-2}\A_{S_{t}}(t)^\top\A_{S_{t}}(t)\right)^{-1}= \F_{S_t}^{-1}
\end{aligned}
\end{equation*}
where $\F_{S_t} = \P_{t|t-1}^{-1}+\sigma^{-2}\sum_{i\in S_{t}}\a_i(t)\a_i(t)^\top$ is the corresponding Fisher information matrix. The MSE at time $t$ is expressed by the trace of the filtered error covariance matrix $\P_{t|t}$. That is, $\mathrm{MSE} = \E\left[{\norm{\x(t)-\hat{\x}_{t|t}}}_2^2\right]= \mathrm{Tr}\left(\F_{S_t}^{-1}\right)$
% \begin{equation}\label{eq:mse}
% \begin{aligned}
% \mathrm{MSE} = \E\left[{\norm{\x(t)-\hat{\x}_{t|t}}}_2^2\right]= \mathrm{Tr}\left(\F_{S_t}^{-1}\right)
% \end{aligned}
% \end{equation}
where $\hat{\x}_{t|t}$ denotes the filtered estimate at time $t$.





==> SimOld.tex <==
To test the performance of the proposed randomized greedy algorithm, we compare it with the classic greedy algorithm and the SDP relaxation in a variety of settings as detailed below. \footnote{MATLAB implementation of the proposed algorithm in this paper is freely available at \url{https://github.com/realabolfazl/RGSS}.}

We consider the problem of Kalman filtering for state estimation in a linear dynamical system. Assume 
%the system is in steady state and 
$\H(t)  = \I_m$ and $\x(0)\sim \mathcal{N}(\mathbf{0},\I_m)$.
%. The initial state is a zero-mean Gaussian random vector with covariance $\mathbf{\Sigma_x} = \I_m$. 
We further specify zero-mean Gaussian process and measurement noises with covariance matrices $\mathbf{Q}=0.05\I_m$ and $\mathbf{R}=0.05\I_n$, respectively. At each time step, the rows of the measurement matrix $\A(t)$, are drawn according to $\mathcal{N} \sim (0,\frac{1}{m}\I_m)$.

The MSE values and running time of each scheme is averaged over 10 Monte-Carlo simulations. The time horizon for each run is $T = 20$. The greedy and randomized greedy algorithms are implemented in MATLAB while the SDP relaxation scheme is implemented via CVX \cite{grant2008cvx}. All experiments were run on a laptop with 2.0 GHz Intel Core i7-4510U CPU and 8.00 GB of RAM.

%===================================
%\subsection{Kalman Filtering over Time}
%===================================
\begin{table}[!htb]
	\centering
	\caption{Running time comparison of randomized greedy, greedy, and SDP relaxation sensor selection schemes.
		%	 ($m=50$, $n=400$, $k=55$, $\epsilon=0.001$).
	}
	\begin{tabular}{|c|c|c|}
		\hline
		Randomized Greedy & Greedy & SDP Relaxation \\ 
		\hline
		0.20 s & 0.38 s & 249.86 s\\
		\hline
	\end{tabular}
	\label{tab:sim1_time}
	%\vspace{-0.3cm}
\end{table}
%===================================
We first consider a system having $m = 50$ states, $n = 400$ measurements, and $k = 55$, and compare the MSE values of each method over the time horizon of interest. For randomized greedy we set $\epsilon = 0.001$. Fig. \oldref{fig:overtime} shows that the greedy method consistently yields the lowest MSE while the MSE of the randomized greedy algorithm is slightly higher. The MSE performance achieved by the SDP relaxation is considerably larger than those of the greedy and randomized greedy algorithms. The running time of each method is given in Table \oldref{tab:sim1_time}. Both the greedy algorithm and the randomized greedy algorithm are much faster than the SDP formulation. The randomized greedy scheme is nearly two times faster than the greedy method.
\begin{figure}[t]
\centering
    \includegraphics[width=0.39\textwidth]{overtimemse}
    \caption{MSE comparison of randomized greedy, greedy, and SDP relaxation sensor selection schemes employed in Kalman filtering.}
\label{fig:overtime}
%\vspace{-0.5cm}
\end{figure}
%Therefore, the randomized greedy outperforms the other two approach in terms of speed while its performance is very close to that of greedy and better than the performance of SDP. 
Note that, in this example, in each iteration of the sensor selection procedure the randomized scheme only computes the marginal gain for a sampled subset of size 50. As a comparison, the greedy approach computes the marginal gain for all 400 sensors. In summary, the greedy method yields the lowest MSE but is much slower than the proposed randomized greedy algorithm.

%===================================
%\subsection{Effect of Number of Selected Sensors}
To study the effect of the number of selected sensors on performance, we vary $k$ from 55 to 115 with increments of 10. The MSE values at the last time step (i.e., $t = 20$) for each algorithm are shown in Fig. \oldref{fig:kvary}(a). As the number of selected sensors increases, the estimation becomes more accurate, as reflected by the MSE of each algorithm. Further, the difference between the MSE values consistently decreases as more sensors are selected. The running times shown in Fig. \oldref{fig:kvary}(b) indicate that the randomized greedy scheme is nearly twice as fast as the greedy method, while the SDP method is orders of magnitude slower than both greedy and randomized greedy algorithms. 
%Hence, for state estimation in large networks, one can achieve state-of-the-art estimation error with significantly lower complexity by employing the proposed randomized greedy algorithm.
%===================================
\begin{figure}[t]
\centering
    \begin{subfigure}{.39\textwidth}
  \centering
    \includegraphics[width=1\textwidth]{systemsizemse}\caption{\scriptsize MSE comparison}
        \end{subfigure}
        \begin{subfigure}{.39\textwidth}
  \centering
    \includegraphics[width=1\textwidth]{systemsizetime}\caption{\scriptsize Running time comparison}
\end{subfigure}
\caption{Comparison of randomized greedy, greedy, and SDP relaxation schemes as the number of selected sensors increases.}
\label{fig:kvary}
%\vspace{-0.6cm}
\end{figure}

%===================================
%\subsection{Effect of System Size}
Finally, we compare the performance of the randomized greedy algorithm to that of the greedy algorithm as the size of the system increases. We run both methods for 20 different sizes of the system. The initial size was set to $m = 20$, $n=200$, and $k=25$ and all three parameters are scaled by $\gamma$ where $\gamma$ varies from 1 to 20. In addition, to evaluate the effect of $\epsilon$ on the performance and runtime of the randomized greedy approach, we repeat experiments for $\epsilon \in \{0.1, 0.01, 0.001\}$.
Note that the computational complexity of the SDP relaxation scheme is prohibitive in this setting. 
Fig. \oldref{fig:betavary}(a) illustrates the percentage difference of the MSE between the two methods. In particular, we show 
\begin{equation*}
\% \: \Delta \mathrm{MSE} = \frac{\mathrm{MSE_{RG}}-\mathrm{MSE_{G}}}{\mathrm{MSE_{G}}} \times 100 
\end{equation*}
where ``RG'' and ``G''  refer to the randomized greedy and greedy algorithms, respectively. It can be seen that this difference between the MSEs reduces as the system scales up.
The running time is plotted in Fig. \oldref{fig:betavary}(b). As the figure illustrates, the gap between the running times grows with the size of the system and the randomized greedy algorithm performs nearly 25 times faster than the greedy method for the largest network.
Fig. \oldref{fig:betavary} shows that using a smaller $\epsilon$ results in a lower MSE  while it slightly increases the running time. These results suggest that, for large systems, the randomized greedy provides almost the same MSE while being much faster than the greedy algorithm.
%===================================
\begin{figure}[t]
\centering
    \begin{subfigure}{.39\textwidth}
  \centering
    \includegraphics[width=1\textwidth]{largescalemse}\caption{\scriptsize $ \Delta \: \mathrm{MSE}$}
        \end{subfigure}
        \begin{subfigure}{.39\textwidth}
  \centering
    \includegraphics[width=1\textwidth]{largescaletime}\caption{\scriptsize Running time comparison}
\end{subfigure}
\caption{A comparison of the randomized greedy and greedy algorithms for varied network size.}
\label{fig:betavary}
%\vspace{-0.7cm}
\end{figure}
